An Expectation Conditional Maximization approach for Gaussian graphical models

Bayesian graphical models are a useful tool for understanding dependence relationships among many variables, particularly in situations with external prior information. In high-dimensional settings, the space of possible graphs becomes enormous, rendering even state-of-the-art Bayesian stochastic search computationally infeasible. We propose a deterministic alternative to estimate Gaussian and Gaussian copula graphical models using an Expectation Conditional Maximization (ECM) algorithm, extending the EM approach from Bayesian variable selection to graphical model estimation. We show that the ECM approach enables fast posterior exploration under a sequence of mixture priors, and can incorporate multiple sources of information.

==> paper-table.tex <==
\begin{table}[htb]

\caption{\label{tab:}Comparing estimation of the AR1 graph for both the Gaussian and non-Gaussian case. Three different sample sizes,  $n = 100$, $200$, and $500$, are compared in the columns.\label{tab:0-1}}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}[t]{cccccccccccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{ } & \multicolumn{3}{c}{Gaussian: F-norm} & \multicolumn{3}{c}{Gaussian: AUC} & \multicolumn{3}{c}{Copula: F-norm} & \multicolumn{3}{c}{Copula: AUC} \\
\cmidrule(l{2pt}r{2pt}){3-5} \cmidrule(l{2pt}r{2pt}){6-8} \cmidrule(l{2pt}r{2pt}){9-11} \cmidrule(l{2pt}r{2pt}){12-14}
p & Method & 100 & 200 & 500 & 100 & 200 & 500 & 100 & 200 & 500 & 100 & 200 & 500\\
\midrule
50 & EMGS & 4.41 & 3.09 & 1.98 & 1 & 1 & 1 & 7.86 & 5.35 & 3.70 & 1 & 1 & 1\\
 & GL-CV & 10.38 & 10.23 & 10.05 & 1 & 1 & 1 & 11.21 & 11.03 & 10.85 & 1 & 1 & 1\\
 & GL-RIC & 17.59 & 15.80 & 13.20 & 1 & 1 & 1 & 17.58 & 15.85 & 13.42 & 1 & 1 & 1\\
 & GL-StARS & 16.49 & 15.27 & 14.50 & 1 & 1 & 1 & 16.87 & 15.72 & 15.01 & 1 & 1 & 1\\
 & GL-rank &  &  &  &  &  &  & 11.14 & 11.00 & 10.84 & 1 & 1 & 1\\
\hline
100 & EMGS & 9.67 & 4.88 & 3.06 & 1 & 1 & 1 & 11.77 & 7.86 & 5.51 & 1 & 1 & 1\\
 & GL-CV & 14.80 & 14.60 & 14.35 & 1 & 1 & 1 & 16.00 & 15.74 & 15.50 & 1 & 1 & 1\\
 & GL-RIC & 26.21 & 23.71 & 20.01 & 1 & 1 & 1 & 25.98 & 23.65 & 20.29 & 1 & 1 & 1\\
 & GL-StARS & 23.07 & 21.14 & 19.84 & 1 & 1 & 1 & 23.58 & 21.82 & 20.59 & 1 & 1 & 1\\
 & GL-rank &  &  &  &  &  &  & 16.87 & 15.72 & 15.49 & 1 & 1 & 1\\
\hline
200 & EMGS & 32.89 & 20.80 & 5.11 & 1 & 1 & 1 & 22.60 & 16.41 & 8.21 & 1 & 1 & 1\\
 & GL-CV & 23.39 & 20.75 & 20.44 & 1 & 1 & 1 & 24.97 & 22.35 & 22.06 & 1 & 1 & 1\\
 & GL-RIC & 38.20 & 34.86 & 29.83 & 1 & 1 & 1 & 37.76 & 34.68 & 30.07 & 1 & 1 & 1\\
 & GL-StARS & 32.31 & 29.54 & 27.57 & 1 & 1 & 1 & 33.10 & 30.65 & 28.82 & 1 & 1 & 1\\
 & GL-rank &  &  &  &  &  &  & 26.50 & 22.34 & 22.06 & 1 & 1 & 1\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htb]

\caption{\label{tab:}Comparing estimation of the AR2 graph for both the Gaussian and non-Gaussian case. Three different sample sizes,  $n = 100$, $200$, and $500$, are compared in the columns.\label{tab:0-2}}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}[t]{cccccccccccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{ } & \multicolumn{3}{c}{Gaussian: F-norm} & \multicolumn{3}{c}{Gaussian: AUC} & \multicolumn{3}{c}{Copula: F-norm} & \multicolumn{3}{c}{Copula: AUC} \\
\cmidrule(l{2pt}r{2pt}){3-5} \cmidrule(l{2pt}r{2pt}){6-8} \cmidrule(l{2pt}r{2pt}){9-11} \cmidrule(l{2pt}r{2pt}){12-14}
p & Method & 100 & 200 & 500 & 100 & 200 & 500 & 100 & 200 & 500 & 100 & 200 & 500\\
\midrule
50 & EMGS & 4.61 & 2.86 & 1.49 & 0.98 & 1.00 & 1.00 & 6.20 & 4.03 & 2.73 & 0.96 & 1.00 & 1.00\\
 & GL-CV & 7.98 & 6.39 & 6.05 & 0.93 & 0.99 & 1.00 & 8.37 & 6.86 & 6.54 & 0.91 & 0.98 & 1.00\\
 & GL-RIC & 12.07 & 11.23 & 9.84 & 0.72 & 0.80 & 0.96 & 11.97 & 11.18 & 9.88 & 0.73 & 0.81 & 0.95\\
 & GL-StARS & 11.54 & 10.95 & 10.56 & 0.77 & 0.83 & 0.89 & 11.64 & 11.10 & 10.72 & 0.76 & 0.81 & 0.86\\
 & GL-rank &  &  &  &  &  &  & 8.96 & 7.25 & 6.83 & 0.90 & 0.98 & 1.00\\
\hline
100 & EMGS & 12.31 & 4.65 & 2.39 & 0.90 & 1.00 & 1.00 & 13.67 & 5.69 & 4.16 & 0.91 & 1.00 & 1.00\\
 & GL-CV & 13.02 & 10.31 & 8.80 & 0.91 & 0.99 & 1.00 & 13.39 & 10.97 & 9.47 & 0.89 & 0.98 & 1.00\\
 & GL-RIC & 17.69 & 16.56 & 14.76 & 0.67 & 0.77 & 0.92 & 17.51 & 16.46 & 14.77 & 0.69 & 0.78 & 0.92\\
 & GL-StARS & 16.38 & 15.51 & 14.83 & 0.78 & 0.84 & 0.92 & 16.54 & 15.71 & 15.08 & 0.77 & 0.83 & 0.89\\
 & GL-rank &  &  &  &  &  &  & 14.13 & 11.84 & 9.88 & 0.87 & 0.97 & 1.00\\
\hline
200 & EMGS & 28.26 & 17.66 & 3.97 & 0.89 & 0.96 & 1.00 & 41.95 & 14.58 & 8.10 & 0.87 & 0.98 & 1.00\\
 & GL-CV & 20.26 & 16.85 & 12.59 & 0.88 & 0.98 & 1.00 & 20.52 & 17.51 & 13.60 & 0.86 & 0.97 & 1.00\\
 & GL-RIC & 25.58 & 24.13 & 21.68 & 0.62 & 0.75 & 0.88 & 25.29 & 23.92 & 21.62 & 0.65 & 0.76 & 0.89\\
 & GL-StARS & 23.21 & 21.97 & 20.93 & 0.79 & 0.85 & 0.94 & 23.43 & 22.26 & 21.32 & 0.77 & 0.84 & 0.91\\
 & GL-rank &  &  &  &  &  &  & 21.47 & 18.62 & 14.72 & 0.84 & 0.95 & 1.00\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htb]

\caption{\label{tab:}Comparing estimation of the random graph for both the Gaussian and non-Gaussian case. Three different sample sizes,  $n = 100$, $200$, and $500$, are compared in the columns.\label{tab:0-3}}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}[t]{cccccccccccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{ } & \multicolumn{3}{c}{Gaussian: F-norm} & \multicolumn{3}{c}{Gaussian: AUC} & \multicolumn{3}{c}{Copula: F-norm} & \multicolumn{3}{c}{Copula: AUC} \\
\cmidrule(l{2pt}r{2pt}){3-5} \cmidrule(l{2pt}r{2pt}){6-8} \cmidrule(l{2pt}r{2pt}){9-11} \cmidrule(l{2pt}r{2pt}){12-14}
p & Method & 100 & 200 & 500 & 100 & 200 & 500 & 100 & 200 & 500 & 100 & 200 & 500\\
\midrule
50 & EMGS & 40.17 & 17.10 & 10.20 & 0.78 & 0.84 & 0.90 & 55.89 & 28.78 & 25.86 & 0.74 & 0.81 & 0.87\\
 & GL-CV & 77.41 & 58.71 & 64.32 & 0.72 & 0.74 & 0.74 & 78.42 & 59.65 & 63.87 & 0.71 & 0.73 & 0.74\\
 & GL-RIC & 84.55 & 63.83 & 66.26 & 0.64 & 0.68 & 0.72 & 84.64 & 64.07 & 65.35 & 0.64 & 0.68 & 0.72\\
 & GL-StARS & 86.86 & 67.76 & 73.92 & 0.60 & 0.61 & 0.60 & 87.20 & 68.02 & 72.73 & 0.59 & 0.60 & 0.59\\
 & GL-rank &  &  &  &  &  &  & 78.67 & 59.90 & 64.16 & 0.71 & 0.73 & 0.73\\
\hline
100 & EMGS & 110.56 & 81.81 & 87.30 & 0.72 & 0.79 & 0.86 & 151.97 & 140.01 & 159.37 & 0.68 & 0.73 & 0.81\\
 & GL-CV & 195.32 & 198.69 & 232.86 & 0.63 & 0.64 & 0.65 & 197.02 & 200.36 & 234.20 & 0.62 & 0.63 & 0.65\\
 & GL-RIC & 207.76 & 208.02 & 236.98 & 0.57 & 0.59 & 0.62 & 207.78 & 208.30 & 237.64 & 0.57 & 0.59 & 0.62\\
 & GL-StARS & 209.52 & 211.85 & 246.98 & 0.55 & 0.56 & 0.56 & 210.84 & 213.46 & 247.66 & 0.55 & 0.55 & 0.55\\
 & GL-rank &  &  &  &  &  &  & 197.33 & 200.74 & 234.64 & 0.62 & 0.63 & 0.64\\
\hline
200 & EMGS & 301.83 & 199.36 & 113.68 & 0.67 & 0.71 & 0.78 & 319.42 & 252.27 & 218.87 & 0.63 & 0.68 & 0.72\\
 & GL-CV & 456.08 & 375.68 & 324.99 & 0.56 & 0.57 & 0.57 & 410.50 & 367.34 & 334.67 & 0.56 & 0.57 & 0.57\\
 & GL-RIC & 475.80 & 392.37 & 335.70 & 0.52 & 0.53 & 0.55 & 427.09 & 379.55 & 343.38 & 0.53 & 0.54 & 0.55\\
 & GL-StARS & 468.35 & 386.38 & 336.51 & 0.54 & 0.54 & 0.54 & 424.00 & 379.34 & 348.51 & 0.53 & 0.54 & 0.53\\
 & GL-rank &  &  &  &  &  &  & 410.83 & 367.84 & 335.20 & 0.56 & 0.56 & 0.57\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htb]

\caption{\label{tab:}Comparing estimation of the cluster graph for both the Gaussian and non-Gaussian case. Three different sample sizes,  $n = 100$, $200$, and $500$, are compared in the columns.\label{tab:0-4}}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}[t]{cccccccccccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{ } & \multicolumn{3}{c}{Gaussian: F-norm} & \multicolumn{3}{c}{Gaussian: AUC} & \multicolumn{3}{c}{Copula: F-norm} & \multicolumn{3}{c}{Copula: AUC} \\
\cmidrule(l{2pt}r{2pt}){3-5} \cmidrule(l{2pt}r{2pt}){6-8} \cmidrule(l{2pt}r{2pt}){9-11} \cmidrule(l{2pt}r{2pt}){12-14}
p & Method & 100 & 200 & 500 & 100 & 200 & 500 & 100 & 200 & 500 & 100 & 200 & 500\\
\midrule
50 & EMGS & 15.05 & 17.64 & 4.16 & 0.87 & 0.90 & 0.93 & 22.36 & 25.16 & 10.29 & 0.85 & 0.89 & 0.92\\
 & GL-CV & 37.53 & 42.95 & 26.04 & 0.86 & 0.88 & 0.90 & 38.25 & 43.63 & 26.70 & 0.85 & 0.88 & 0.90\\
 & GL-RIC & 43.08 & 47.11 & 27.88 & 0.79 & 0.83 & 0.87 & 42.97 & 47.17 & 28.18 & 0.79 & 0.83 & 0.87\\
 & GL-StARS & 42.04 & 46.71 & 29.00 & 0.82 & 0.84 & 0.85 & 42.39 & 47.08 & 29.45 & 0.81 & 0.83 & 0.85\\
 & GL-rank &  &  &  &  &  &  & 38.56 & 43.85 & 26.94 & 0.85 & 0.87 & 0.90\\
\hline
100 & EMGS & 73.72 & 10.29 & 34.66 & 0.86 & 0.90 & 0.93 & 85.92 & 16.66 & 61.58 & 0.85 & 0.88 & 0.92\\
 & GL-CV & 108.50 & 37.63 & 97.04 & 0.85 & 0.88 & 0.89 & 109.56 & 38.59 & 98.15 & 0.84 & 0.87 & 0.89\\
 & GL-RIC & 116.97 & 44.42 & 100.86 & 0.77 & 0.81 & 0.86 & 116.81 & 44.36 & 101.28 & 0.78 & 0.82 & 0.87\\
 & GL-StARS & 114.52 & 42.42 & 101.34 & 0.81 & 0.84 & 0.85 & 115.04 & 43.02 & 101.78 & 0.81 & 0.84 & 0.86\\
 & GL-rank &  &  &  &  &  &  & 110.13 & 38.92 & 98.51 & 0.84 & 0.87 & 0.89\\
\hline
200 & EMGS & 138.88 & 34.82 & 25.10 & 0.85 & 0.90 & 0.94 & 157.46 & 37.31 & 37.15 & 0.84 & 0.89 & 0.93\\
 & GL-CV & 165.99 & 84.30 & 104.89 & 0.84 & 0.88 & 0.90 & 167.19 & 69.77 & 84.09 & 0.84 & 0.88 & 0.90\\
 & GL-RIC & 176.58 & 94.91 & 111.59 & 0.74 & 0.81 & 0.86 & 176.23 & 78.70 & 89.45 & 0.75 & 0.81 & 0.86\\
 & GL-StARS & 172.47 & 90.83 & 110.32 & 0.81 & 0.84 & 0.86 & 173.14 & 75.59 & 88.50 & 0.80 & 0.84 & 0.86\\
 & GL-rank &  &  &  &  &  &  & 168.42 & 70.40 & 84.55 & 0.84 & 0.87 & 0.89\\
\bottomrule
\end{tabular}
\end{table}

